Inhabitation for Non-idempotent Intersection Types

The inhabitation problem for intersection types in the lambda-calculus is known to be undecidable. We study the problem in the case of non-idempotent intersection, considering several type assignment systems, which characterize the solvable or the strongly normalizing lambda-terms. We prove the decidability of the inhabitation problem for all the systems considered, by providing sound and complete inhabitation algorithms for them.

==> macros.tex <==
\long\def\ignore#1{\relax}
%\newtheorem{defi}{Definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{property}{Property}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{notation}[theorem]{Notation}
%\newcommand{\PROOF}[1]{{\em Proof. }#1{ $\qquad \diamond $ \medskip}}
%\newcommand{\proof}[1]{{\em Proof. } #1 { $\diamond $}}
%\renewenvironment{proof}{{\em Proof. }}{\hfill $\diamond$}

%\def\proof{\par\addvspace{5pt}\trivlist\item[\hskip\labelsep{\it Proof.}]}
%%%%%%%%SYNTAX
\newcommand{\s}{{\tt t}}
\newcommand{\uu}{{\tt u}}
\newcommand{\vv}{{\tt v}}
\newcommand{\x}{{\tt x}}
\newcommand{\y}{{\tt y}}
\newcommand{\z}{{\tt z}}
\newcommand{\w}{{\tt w}}
\newcommand{\ap}{{\tt a}}
\newcommand{\bp}{{\tt b}}
\newcommand{\cp}{{\tt c}}
\newcommand{\iid}{{\tt I}}
\newcommand{\dup}{{\tt D}}
\newcommand{\Ap}{{\mathcal A}}
\newcommand{\Lp}{{\Lambda_p}}
\newcommand{\Llp}{{\Lambda_\pi}}
\newcommand{\proj}[1]{\pi_{#1}}
\newcommand{\sproj}{\overline\pi}
\newcommand{\sprojp}{\overline{ \pi '}}
\newcommand{\ssproj}{\mathtt{P}_{\overline \pi}}
\newcommand{\ssprojp}{\mathtt{P}_{\overline \pi'}}
\newcommand{\sterm}[1]{\overline{#1}}
\newcommand{\Lop}{{\Lambda^{\Omega}_p}}
\newcommand{\true}{{\tt  true}}
\newcommand{\false}{{\tt  false}}
\newcommand{\p}{{\tt p}}
\newcommand{\q}{{\tt q}}
\newcommand{\Rew}[1]{\rightarrow_{#1}}
\newcommand{\LRew}[1]{\mbox{}_{#1} \!\! \leftarrow}
\newcommand{\Rewn}[1]{\rightarrow^*_{#1}}
\newcommand{\Rewplus}[1]{\rightarrow^+_{#1}}
\newcommand{\bg}{\beta g}
\newcommand{\nf}{{\tt nf}}
\newcommand{\hnf}{{\tt hnf}}
\newcommand{\canf}{{\em cnf}}
\newcommand{\HN}{{\em HNF}}
\newcommand{\CF}{{\em CNF}}
\newcommand{\redi}{\rightarrow_i}
\newcommand{\redis}{\rightarrow^*_i}
\newcommand{\red}{\rightarrow}
\newcommand{\reds}{\rightarrow^*}
\newcommand{\redb}{\rightarrow_{\beta}}
\newcommand{\redo}{\rightarrow_{\beta\omega}}
\newcommand{\redh}{\rightarrow_{h}}
\newcommand{\redhs}{\rightarrow^{*}_{h}}
\newcommand{\redsafe}{\rightarrow_{s}}
\newcommand{\redsafes}{\rightarrow^*_{s}}
\newcommand{\redsh}{\rightarrow_{sh}}
\newcommand{\redshs}{\rightarrow^*_{sh}}
\newcommand{\redbs}{\rightarrow^{*}_{\beta}}
\newcommand{\redp}{\rightarrow_{\pi}}
\newcommand{\redps}{\rightarrow^{*}_{\pi}}
\newcommand{\redhp}{\rightarrow^{h}_{\pi}}
\newcommand{\redzero}{\rightarrow_{0}}
%\newcommand{\conv}{\Downarrow}
\newcommand{\ddiv}{\Uparrow}
\newcommand{\cond}{\mathcal  C}
\newcommand{\err}{\star}
\newcommand{\pair}[2]{\langle #1,#2 \rangle }

%%%%%%%SEMANTICS
\newcommand{\solv}{SOLV}
\newcommand{\sat}{SAT}
\newcommand{\satf}{SAT_\arrow}
\newcommand{\sati}[1]{SAT^{#1}_\times}
\newcommand{\satl}{SAT^1_\times}
\newcommand{\satr}{SAT^2_\times}
\newcommand{\sato}{\Omega}

%denotational sematics
%
\newcommand{\dpap}{[\![}
\newcommand{\dpch}{]\!]}

%den e' la funzione di interpretazione semantica
\newcommand{\den}[1]{\dpap {#1} \dpch}

%dene e' la funzione di interpretazione semantica in un environment
\newcommand{\dene}[2]{\dpap {#1} \dpch _{#2}}


%%%%%%TYPES
\newcommand{\A}{{\tt A}}
\newcommand{\D}{{\tt B}}
\newcommand{\arrow}{\rightarrow}
\newcommand{\inter}{\wedge}
\newcommand{\Inter}{ \bigwedge}
\newcommand{\iset}[1]{\{#1\}}
\newcommand{\der}{\vdash}
\newcommand{\ders}{\vdash_{{\footnotesize \Su}}}
\newcommand{\derss}{\vdash_{\footnotesize \Su,\leq}}
\newcommand{\derw}{\vdash_{\footnotesize w}}
\newcommand{\oder}{\vdash_{\Omega}}
\newcommand{\dero}{\vdash_\Omega}
\newcommand{\pdero}{\Vdash_\Omega}
\newcommand{\dert}{\vdash^{*}}
\newcommand{\union}{\odot  }
\newcommand{\comp}{{\tt  comp}}
\newcommand{\T}{\mathcal T}
\newcommand{\TM}{{\mathcal{TM}}}
\newcommand{\TP}{{\mathcal{TP}}}
\newcommand{\match}[1]{\ll^{#1}}
\newcommand{\sep}{\hspace{.5cm}}
\newcommand{\Mu}{\mathcal H}
\newcommand{\Pu}{\mathcal P}
\newcommand{\Su}{\mathcal S}
\newcommand{\Pus}{\mathcal P_{s}}
\newcommand{\Puw}{\mathcal P_{w}}
\newcommand{\Pul}{\mathcal P_{l}}
\newcommand{\dem}{\triangleright}
%%%%%%%%
%%%%%%%%%COMMENTI


\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\violet}[1]{\textcolor{Plum}{#1}}
\newcommand{\rose}[1]{\textcolor{Magenta}{#1}}
\newcommand{\rouge}[1]{{\color{red} #1}}
\newcommand{\green}[1]{{\color{beauvert} #1}}

\newcommand{\CS}[1]{{ \color{red} {\bf{SiC}} #1 }}
\newcommand{\CD}[1]{{ \color{Plum} {\bf{DeC}} #1 }}
\newcommand{\CDA}[1]{{ \color{red} { {\bf{DeAnC}} #1 }}}
\newcommand{\CAN}[1]{{ \color{red} { #1 }}}
\newcommand{\changed}[2]{{ \color{Plum} { {\bf{DC}} #2 }}} 
\newcommand{\changea}[2]{\violet{{\bf AnChange }#2}}
\newcommand{\changeda}[2]{{ \color{red} { {\bf{DeAnC}} #2 }}} 
\newcommand{\changeds}[2]{{ \color{blue} { {\bf{SiChange}} #2 }}} 
\newcommand{\CA}[1]{\violet{{\bf AnC }#1 }}
\newcommand{\multiset}[1]{[#1]}
\newcommand{\mmult}[1]{[ \! [ #1 ] \! ]}
\newcommand{\emul}{\multiset{\, }}
\newcommand{\set}[1]{\{ #1 \}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ih}{{\it i.h.}}
\newcommand{\isubs}[2]{\{ #1 / #2 \}}
\newcommand{\qsub}[3]{#1[#2\leftarrow #3]}
\newcommand{\Gam}{\Gamma}
\newcommand{\Sig}{\Sigma}

\newcommand{\Del}{\Delta}
\newcommand{\del}{\del}
\newcommand{\gam}{\gamma}

\newcommand{\fv}[1]{{\tt fv}(#1)}
\newcommand{\bv}[1]{{\tt bv}(#1)}
\newcommand{\var}[1]{{\tt var}(#1)}
\newcommand{\dom}[1]{{\tt dom}(#1)}
\newcommand{\codom}[1]{{\tt codom}(#1)}
\newcommand{\st}{\, | \,}
\newcommand{\prodmul}{\mathbb{X}}
\newcommand{\com}[1]{{\tt DC}(#1)}
\newcommand{\comt}[1]{{\tt TC}(#1)}
\newcommand{\omegaprod}{\omega_{\times}}
\newcommand{\omegaf}{\omega_{\arrow}}
\newcommand{\pathu}{\times_{1}}
\newcommand{\pathd}[1]{\times_{2}}
\newcommand{\prodi}[2]{\times_{#2}(#1)}
\newcommand{\produ}[1]{\times_1(#1)}
\newcommand{\prodd}[1]{\times_2(#1)}
\newcommand{\produt}{\times_{1}}
\newcommand{\proddt}{\times_{2}}
\newcommand{\prodp}[2]{\times_{#1}(#2)}
\newcommand{\prodpt}[1]{\times_{#1}}
%\newcommand{\pder}[1]{\Vdash_{#1}}
\newcommand{\pderr}{\Vdash_\res}
\newcommand{\pders}{\Vdash_\str}
\newcommand{\res}{{\tt r}}
\newcommand{\str}{{\tt s}}

\newcommand{\pder}{\Vdash}
\newcommand{\sm}{\setminus}
\newcommand{\Set}{{\cal S}}
\newcommand{\tat}[2]{#1(#2)}
\newcommand{\regla}[3]{
    \prooftree
         #1
    \justifies  
         #2
    \thickness=0.05em
    \using
        #3
    \endprooftree}
\newcommand{\hred}{\Rew{h}}
\newcommand{\hredn}{\Rewn{h}}
\newcommand{\ired}{\Rew{i}}
\newcommand{\hRedP}[1]{\ensuremath{\underset{#1}{\rightsquigarrow}}}
\newcommand{\matches}[3]{\ensuremath{{#1}\ll^{#3}{#2}}}
\newcommand{\es}{\emptyset}
\newcommand{\msum}[3]{\sum_{#1}^{#2} #3}
\newcommand{\et}[1]{(#1)^*}
\def\l{\lambda}
\newcommand{\redk}{\Rew{K}}
\newcommand{\redsk}{\Rewn{K}}
\newcommand{\slist}{{\tt L}}
\newcommand{\mlist}{{\tt M}}
\newcommand{\id}{{\tt I}}
\newcommand{\fail}{{\tt fail}}
\newcommand{\deft}[1]{{\bf #1}}
\newcommand{\nil}{{\tt nil}}
\newcommand{\tri}[3]{\langle #1, #2, #3 \rangle}
\newcommand{\size}[1]{{ \tt size}(#1)}
\newcommand{\cpx}[1]{{ \tt cpx}(#1)}
\newcommand{\run}{r_1}
\newcommand{\rdeux}{r_2}
\newcommand{\rtrois}{r_3}
\newcommand{\rquatre}{r_6}
\newcommand{\rcinq}{r_7}
\newcommand{\rsix}{r_8}
\newcommand{\rsept}{r_9}
\newcommand{\rhuit}{r_{10}}
\newcommand{\rneuf}{r_{11}}
\newcommand{\rdix}{r_{4}}
\newcommand{\ronze}{r_{5}}

\newcommand{\App}{{\cal A}}
\newcommand{\B}{{\cal B}}
\newcommand{\I}{{\cal I}}
\newcommand{\J}{{\cal J}}

%\newcommand{\Reweq}[1]{\Rew{#1}^{=}}
\newcommand{\Reweq}[1]{\stackrel{=}{\Rew{#1}}}
\newcommand{\sig}{\sigma}
\newcommand{\meaningful}{meaningful}
\newcommand{\canonical}{canonical form}
\newcommand{\Canonical}{Canonical form}
\newcommand{\mean}{meaningful}
\renewcommand{\approx}{approximate form}
\newcommand{\headset}{head-set}
\newcommand{\can}{{\bf cf}}
\newcommand{\mcan}{{\bf mcf}}
\newcommand{\lift}[1]{\uparrow \!\!  (#1)}
\newcommand{\listpatterns}[1]{\overline{#1}}
\newcommand{\longproof}[1]{\ignore{#1}}
%\newcommand{\antonio}[1]{{\color{magenta} {#1}}}
%\newcommand{\cantonio}[2]{{\antonio{#2}}}

%\newcommand{\simona}[1]{{\color{red} {#1}}}
%\newcommand{\delia}[1]{{\color{blue} {#1}}}
%\newcommand{\bdelia}[1]{\sout{{\delia{#1}}}}
%\newcommand{\bsimona}[1]{\sout{{\simona{#1}}}}
%\newcommand{\cdelia}[2]{{\delia{#2}}}

\newcommand{\cwc}[1]{[ \! \! [ #1 ] \! \! ]} 
\newcommand{\ccontext}{{\tt C}}
\newcommand{\hcontext}{{\tt H}}
\newcommand{\dermul}{\triangleright}
\newcommand{\inh}{\, \Box \, }
\newcommand{\inhm}{\, \boxdot \, }
\newcommand{\inhp}{\, \triangleright \, }


\newcommand{\ccount}[1]{\#(#1)} 
\newcommand{\iI}{i \in I}
\newcommand{\jJ}{j \in J}
\newcommand{\kK}{k  \in K}
\newcommand{\mM}{m  \in M}

\newcommand{\ex}[1]{{\tt E}(#1)}
\newcommand{\de}[1]{{\tt D}(#1)}
\newcommand{\un}[1]{{\tt U}(#1)}
\newcommand{\bu}{\bigvee}
\newcommand{\C}{{\tt C}}


%\newcommand{\Lp}{\Lambda_{P}}
\newcommand{\LO}{\Lambda_{\Omega}}
\newcommand{\fin}[1]{{\tt F}(#1)}
\newcommand{\lis}[1]{{\tt L}(#1)}
\newcommand{\el}{\langle \, \rangle}
\newcommand{\cons}[2]{#1 :: #2}
\newcommand{\donne}{\triangleright}


\newcommand{\varpat}{{\tt Varpat}}
\newcommand{\weakpat}{{\tt Weakpat}}
\newcommand{\Final}{{\tt Final}}
\newcommand{\Head}{{\tt Head}}
\newcommand{\Headu}{{\tt Head1}}
\newcommand{\Headd}{{\tt Head2}}
\newcommand{\Prefix}{{\tt Prefix}}
\newcommand{\Abs}{{\tt Abs}}
\newcommand{\Union}{{\tt Union}}
\newcommand{\Unionk}{{\tt TUnion}}
\newcommand{\Unionl}{{\tt HUnion}}
\newcommand{\Ome}{{\tt Omega}}
\newcommand{\Pair}{{\tt Pair}}
\newcommand{\Produ}{{\tt Prod1}}
\newcommand{\Prodd}{{\tt Prod2}}
\newcommand{\Proj}{{\tt Proj}}
\newcommand{\Subs}{{\tt Subs}}
\newcommand{\Env}{{\tt Env}}

\newcommand{\Pa}[2]{{\tt P}^{#1}_{#2}}
\newcommand{\K}{{\tt T}}
\newcommand{\M}{{\tt E}}
\newcommand{\KI}{{\tt TI}}
\newcommand{\LK}[2]{{\tt H}_{#1}^{#2}}
\newcommand{\LKI}[2]{{\tt HI}_{#1}^{#2}}
\newcommand{\V}{{\cal V}}
\newcommand{\meas}{{\tt meas}}
\newcommand{\rond}[1]{{#1}^\circ}
%\newcommand{\alt}{{\cal A}}
\newcommand{\altp}{{\cal A}_0}
\newcommand{\ov}[1]{\overline{#1}}




\newcommand{\redpat}{{\cal B}}
\newcommand{\regle}[1]{r{#1}}
\newcommand{\borne}{\triangledown}
\newcommand{\R}{{\ca R}}
\renewcommand{\S}{{\cal S}}
%\newcommand{\str}[1]{{\tt st}(#1)}
\newcommand{\multisetunion}{\sqcup}

\newcommand{\prodr}{\mathbb{X}_\res}
\newcommand{\prods}{\mathbb{X}_\str}
\newcommand{\struc}[1]{{\cal S}(#1)}
\newcommand{\structype}[2]{{\cal S}_{#2}(#1)}
%\newcommand{\support}[1]{{\cal 
\newcommand{\occ}[1]{\mathtt{o}(#1)}
\newcommand{\tocc}[1]{\mathtt{to}(#1)}
\newcommand{\pc}{\nabla}
\newcommand{\sem}[2]{[\![#1]\!]#2} 

\newcommand{\ems}{\multiset{\;}}
\newcommand{\axvar}{\mathtt{var}}
\newcommand{\axvarw}{\mathtt{var}_w}
\newcommand{\arri}{\mathtt{\arrow_{I}}}
\newcommand{\arrie}{\mathtt{\arrow_{I\multiset{}}}}
\newcommand{\arrine}{\mathtt{\arrow_{I\not\multiset{}}}}
\newcommand{\arre}{\mathtt{\arrow_{E}}}
\newcommand{\arree}{\mathtt{\arrow_{E\multiset{}}}}
\newcommand{\arrene}{\mathtt{\arrow_{E\not\multiset{}}}}
\newcommand{\inti}{\mathtt{\wedge_{I}}}
\newcommand{\inte}{\mathtt{\wedge_{E}}}
\newcommand{\many}{\mathtt{m}}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "final.tex"
%%% End:

